A Second-Order Perspective on Model Compositionality and Incremental Learning

The fine-tuning of deep pre-trained models has revealed compositional properties, with multiple specialized modules that can be arbitrarily composed into a single, multi-task model. However, identifying the conditions that promote compositionality remains an open issue, with recent efforts concentrating mainly on linearized networks. We conduct a theoretical study that attempts to demystify compositionality in standard non-linear networks through the second-order Taylor approximation of the loss function. The proposed formulation highlights the importance of staying within the pre-training basin to achieve composable modules. Moreover, it provides the basis for two dual incremental training algorithms: the one from the perspective of multiple models trained individually, while the other aims to optimize the composed model as a whole. We probe their application in incremental classification tasks and highlight some valuable skills. In fact, the pool of incrementally learned modules not only supports the creation of an effective multi-task model but also enables unlearning and specialization in certain tasks. Code available at https://github.com/aimagelab/mammoth.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/awesome.tex <==
%\noindent\textbf{Lore}: \textdagger
%
\tit{General}
\begin{enumerate}[label=1\alph*., leftmargin=0.3in]
    \item \qmarks{Deep Model Fusion: A Survey}~\cite{li2023deep} (2023, China) \linkarxiv{https://arxiv.org/abs/2309.15698}
    \item \qmarks{Modular Deep Learning}~\cite{pfeiffer2023modular} (2024, DeepMind) \linkarxiv{https://arxiv.org/abs/2302.11529}
    \item \qmarks{To Stay or Not to Stay in the Pre-train Basin: Insights on Ensembling in Transfer Learning}~\cite{sadrtdinov2024stay} (NEURIPS 23, Munich) \linkarxiv{https://arxiv.org/abs/2303.03374}
    \item \qmarks{Learning useful representations for shifting tasks and distributions}~\cite{zhang2023learning} (ICML 23, Facebook) \linkarxiv{https://arxiv.org/abs/2212.07346}
    \item \qmarks{Joint Training of Deep Ensembles Fails Due to Learner Collusion}~\cite{jeffares2024joint} (NEURIPS 23, Cambridge) \linkarxiv{https://arxiv.org/abs/2301.11323}
    \item \qmarks{Does Combining Parameter-efficient Modules Improve Few-shot Transfer Accuracy?}~\cite{asadi2024does} (2024, Huawei) \linkarxiv{https://arxiv.org/abs/2402.15414}
    \item \qmarks{Fine-Tuning Can Distort Pretrained Features And Underperform Out-Of-Distribution}~\cite{kumar2022fine} (ICLR 22, Stanford) \linkarxiv{https://arxiv.org/abs/2202.10054}
    \item \qmarks{Understanding the Role of Training Regimes in Continual Learning}~\cite{mirzadeh2020understanding} (NEURIPS 20, Deep Mind \& Washington) \linkarxiv{https://arxiv.org/abs/2006.06958}
\end{enumerate}
%
\tit{Model soup}
\begin{enumerate}[label=2\alph*., leftmargin=0.3in]
    \item \qmarks{Model soups: averaging weights of multiple fine-tuned models improves accuracy without increasing inference time}~\cite{wortsman2022model} (ICML 22, Washington \& Google \& Meta) \linkarxiv{https://arxiv.org/abs/2203.05482}
    \item \qmarks{Merging Models with Fisher-Weighted Averaging}~\cite{matena2022merging} (NEURIPS 22, North Carolina) \linkarxiv{https://arxiv.org/abs/2111.09832}
    \item \qmarks{AdapterSoup: Weight Averaging to Improve Generalization of Pretrained Language Models}~\cite{chronopoulou2023adaptersoup} (EACL 23, Munich) \linkarxiv{https://arxiv.org/abs/2302.07027}
    \item \qmarks{TIES-MERGING: Resolving Interference When Merging Models}~\cite{yadav2024ties} (NEURIPS 23, North Carolina \& IBM \& MIT) \linkarxiv{https://arxiv.org/abs/2306.01708}
    \item \qmarks{Dataless Knowledge Fusion By Merging Weights Of Language Models}~\cite{jin2022dataless} (ICLR 23, Southern California \& Bloomberg) \linkarxiv{https://arxiv.org/abs/2212.09849}
    \item \qmarks{Trainable Weight Averaging: Efficient Training By Optimizing Historical Solutions}~\cite{li2022trainable} (ICLR 23, China) \linkarxiv{https://openreview.net/pdf?id=8wbnpOJY-f}
    \item \qmarks{Model Merging by Uncertainty-Based Gradient Matching}~\cite{daheim2023model} (ICLR 24, UKP Lab) \linkarxiv{https://arxiv.org/abs/2310.12808} (ICLR 24)
    \item \qmarks{Zipit! merging models from different tasks without training}~\cite{stoica2023zipit} (ICLR 2024, Georgia Tech) \linkarxiv{https://arxiv.org/abs/2305.03053} \textdagger
    \item \qmarks{PopulAtion Parameter Averaging (PAPA)}~\cite{jolicoeur2023population} (2023, Samsung) \linkarxiv{https://arxiv.org/abs/2304.03094}
    \item \qmarks{Merging by Matching Models in Task Subspaces}~\cite{tam2023merging} (2024, Toronto \& North Carolina) \linkarxiv{https://arxiv.org/abs/2312.04339}
    \item \qmarks{Trainable Weight Averaging: A General Approach for Subspace Training}~\cite{li2022trainable} (2023, China) \linkarxiv{https://arxiv.org/abs/2205.13104}
    \item \qmarks{Knowledge Fusion Of Large Language Models}~\cite{wan2024knowledge}  (ICLR 24, China) \linkarxiv{https://arxiv.org/abs/2401.10491}
\end{enumerate}
%
\tit{Task-Arithmetic}
\begin{enumerate}[label=3\alph*., leftmargin=0.3in]
    \item \qmarks{Editing Models With Task Arithmetic}~\cite{ilharco2022editing} (ICLR 23, Washington \& Microsoft) \linkarxiv{https://arxiv.org/abs/2212.04089}
    \item \qmarks{Elastic Weight Removal for Faithful and Abstractive Dialogue Generation}~\cite{daheim2023elastic} (2023, ETH \& Edimburgo) \linkarxiv{https://arxiv.org/abs/2303.17574}
    \item \qmarks{Localizing Task Information for Improved Model Merging and Compression}~\cite{wang2024localizing} (ICML 2024, EPFL)
    \item \qmarks{Patching open-vocabulary models by interpolating weights}~\cite{ilharco2022patching} (NEURIPS 2022) \linkarxiv{https://arxiv.org/abs/2208.05592}
\end{enumerate}
%
\tit{Linearized Models}
\begin{enumerate}[label=4\alph*., leftmargin=0.3in]
    \item \qmarks{A Kernel-Based View of Language Model Fine-Tuning}~\cite{malladi2023kernel} (ICML 23, Princeton) \linkarxiv{https://arxiv.org/abs/2210.05643}
    \item \qmarks{Task Arithmetic in the Tangent Space: Improved Editing of Pre-Trained Models}~\cite{ortiz2024task} (NEURIPS 23, EPFL) \linkarxiv{https://arxiv.org/abs/2305.12827}
    \item \qmarks{Tangent Model Composition for Ensembling and Continual Fine-tuning}~\cite{liu2023tangent} (ICCV 23, California) \linkarxiv{https://arxiv.org/abs/2307.08114}
    \item \qmarks{Parameter Efficient Multi-task Model Fusion with Partial Linearization}~\cite{tang2023parameter} (ICLR 24, China) \linkarxiv{https://arxiv.org/abs/2310.04742}
    \item \qmarks{Tangent transformers for composition, privacy and removal}~\cite{liu2023tangenttransformers} (ICLR 24, California) \linkarxiv{https://arxiv.org/abs/2307.08122}
    \item \qmarks{On the Emergence of Cross-Task Linearity in the Pretraining-Finetuning Paradigm}~\cite{zhou2024cross} (2024, China \& California) \linkarxiv{https://arxiv.org/abs/2402.03660}
    \item \qmarks{What can linearized neural networks actually say about generalization?}~\cite{ortiz2021can} (NEURIPS 21, EPFL) \linkarxiv{https://arxiv.org/abs/2106.06770}
\end{enumerate}
%
\tit{Low-Rank tuning and Composable Models}
\begin{enumerate}[label=5\alph*., leftmargin=0.3in]
    \item \qmarks{Composing Parameter-Efficient Modules with Arithmetic Operations}~\cite{zhang2024composing} (NEURIPS 2023, China) \linkarxiv{https://arxiv.org/abs/2306.14870}
    \item \qmarks{Lorahub: Efficient cross-task generalization via dynamic lora composition}~\cite{huang2023lorahub} (REJECT, ICLR 24, Sea AI Lab \& Washington) \linkarxiv{https://arxiv.org/abs/2307.13269}
    \item \qmarks{MoLE: Mixture of LoRA Experts}~\cite{wu2023mole} (ICLR 24) \linkarxiv{https://openreview.net/forum?id=uWvKBCYh4S}
    \item \qmarks{LoRA Training in the NTK Regime has No Spurious Local Minima}~\cite{jang2024lora} (2024, Seoul \& Princeton) \linkarxiv{https://arxiv.org/abs/2402.11867}
    \item \qmarks{Training Neural Networks from Scratch with Parallel Low-Rank Adapters}~\cite{huh2024training} (REJECT, ICLR 24, MIT) \linkarxiv{https://arxiv.org/abs/2402.16828}
    \item \qmarks{Adamix: Mixture-of-adapter For Parameter-efficient Tuning Of Large Language Models}~\cite{wang2022adamix} (EMNLP 2022, Microsoft) \linkarxiv{https://arxiv.org/abs/2205.12410}
\end{enumerate}
%
\tit{Prompt tuning and Composable Models}
\begin{enumerate}[label=6\alph*., leftmargin=0.3in]
    \item \qmarks{A-la-carte prompt tuning (apt): Combining distinct data via composable prompting}~\cite{bowman2023carte} (CVPR 23, AWS \& California) \linkarxiv{https://arxiv.org/abs/2302.07994}
    \item \qmarks{Hierarchical Prompt Learning for Multi-Task Learning}~\cite{liu2023hierarchical} (CVPR 23, China) \linkarxiv{https://openaccess.thecvf.com/content/CVPR2023/papers/Liu_Hierarchical_Prompt_Learning_for_Multi-Task_Learning_CVPR_2023_paper.pdf}
    \item \qmarks{Prompt Algebra for Task Composition}~\cite{perera2023prompt} (2023, AWS) \linkarxiv{https://arxiv.org/abs/2306.00310}
\end{enumerate}
%
\tit{Applications to Continual Leaning}
\begin{enumerate}[label=7\alph*., leftmargin=0.3in]
    \item \qmarks{Task Arithmetic with LoRA for Continual Learning}~\cite{chitale2023task} (NEURIPS 23 Workshop, India) \linkarxiv{https://arxiv.org/abs/2311.02428}
    \item \qmarks{Integral Continual Learning Along the Tangent Vector Field of Tasks}~\cite{liu2022integral} (2023, California \& AWS) \linkarxiv{https://arxiv.org/abs/2211.13108}
    \item \qmarks{Preventing Zero-Shot Transfer Degradation in Continual Learning of Vision-Language Models}~\cite{zheng2023preventing} (ICCV 23, Berkeley \& China) \linkarxiv{https://arxiv.org/abs/2303.06628}
    \item \qmarks{Continual Learning in Low-rank Orthogonal Subspaces}~\cite{chaudhry2020continual} (NEURIPS 20, Oxford) \linkarxiv{https://arxiv.org/abs/2010.11635}
    \item \qmarks{Overcoming Generic Knowledge Loss With Selective Parameter Update}~\cite{zhang2023overcoming} (submitted to ICLR 24, Aljundi) \linkarxiv{https://openreview.net/pdf?id=n8UYBYE9SQ}
    \item \qmarks{Divide And Not Forget: Ensemble Of Selectively Trained Experts In Continual Learning}~\cite{rypesc2024divide} (ICLR 24, Barcelona) \linkarxiv{https://arxiv.org/abs/2401.10191}
\end{enumerate}
%
\tit{Useful}
%
\begin{enumerate}[label=8\alph*., leftmargin=0.3in]
    \item \qmarks{Online Structured Laplace Approximations For Overcoming Catastrophic Forgetting}~\cite{ritter2018online} (University College London) \linkarxiv{https://arxiv.org/abs/1805.07810}
    \item \qmarks{Few-Shot Parameter-Efficient Fine-Tuning is Better and Cheaper than In-Context Learning}~\cite{liu2022few} (NEURIPS 22, North Carolina) \linkarxiv{https://arxiv.org/pdf/2205.05638}
    \item \qmarks{BitFit: Simple Parameter-efficient Fine-tuning for Transformer-based Masked Language-models}~\cite{zaken2021bitfit} (ACL 2022, Allen Institute) \linkarxiv{https://arxiv.org/abs/2106.10199}
    \item \qmarks{Tied-Lora: Enhancing parameter efficiency of LoRA with weight tying}~\cite{renduchintala2023tied} (NVIDIA) \linkarxiv{https://arxiv.org/abs/2311.09578}
    \item \qmarks{VeRA: Vector-based Random Matrix Adaptation}~\cite{kopiczko2023vera} (ICLR 24, Qualcomm) \linkarxiv{https://arxiv.org/abs/2310.11454}
    \item \qmarks{Conditional Adapters: Parameter-efficient
Transfer Learning with Fast Inference}~\cite{lei2024conditional} (NEURIPS 23, Google) \linkarxiv{https://arxiv.org/abs/2304.04947}
    \item \qmarks{Parameter-Efficient Orthogonal Finetuning via Butterfly Factorization}~\cite{liu2023parameter} (ICLR 2024, Max-Planck \& ETH) \linkarxiv{https://openreview.net/pdf?id=7NzgkEdGyr}
\end{enumerate}

